Episode Adaptive Embedding Networks for Few-shot Learning

Few-shot learning aims to learn a classifier using a few labelled instances for each class. Metric-learning approaches for few-shot learning embed instances into a high-dimensional space and conduct classification based on distances among instance embeddings. However, such instance embeddings are usually shared across all episodes and thus lack the discriminative power to generalize classifiers according to episode-specific features. In this paper, we propose a novel approach, namely \emph{Episode Adaptive Embedding Network} (EAEN), to learn episode-specific embeddings of instances. By leveraging the probability distributions of all instances in an episode at each channel-pixel embedding dimension, EAEN can not only alleviate the overfitting issue encountered in few-shot learning tasks, but also capture discriminative features specific to an episode. To empirically verify the effectiveness and robustness of EAEN, we have conducted extensive experiments on three widely used benchmark datasets, under various combinations of different generic embedding backbones and different classifiers. The results show that EAEN significantly improves classification accuracy about $10\%$ to $20\%$ in different settings over the state-of-the-art methods.

==> files/abstract.tex <==
Few-shot learning aims to learn a classifier with limited labeled data, where the classifier is trained on instances of seen classes and generalizes to classify instances from novelty unseen classes. The episode training strategy usually embeds instances to a high-dimensional space and conduct classification in this space. 
Ideally, instance embeddings should be specific and discriminate for an episode. However, generic embeddings of instances are shared across all episodes in most works. In this paper, we propose a novel approach, namely \emph{Episode Adaptive Embedding Networks} (EAENs), to learn episode-specific embeddings of instances. It linearly maps generic embeddings to episode specific embeddings of instances. The map function is learnt from the distribution of generic embeddings of all instances at each dimension. In addition, EAEN can easily combine different generic embedding backbones and different classifiers. We conduct experiments on three widely used benchmark datasets for few-shot learning to show the effectiveness and robustness of EAEN. The experimental results show that the EAEN can greatly improve classification accuracy about $10\%$ to $20\%$ in different settings compared with the state-of-the-art methods.
